A new class of metrics for learning on real-valued and structured data

We propose a new class of metrics on sets, vectors, and functions that can be used in various stages of data mining, including exploratory data analysis, learning, and result interpretation. These new distance functions unify and generalize some of the popular metrics, such as the Jaccard and bag distances on sets, Manhattan distance on vector spaces, and Marczewski-Steinhaus distance on integrable functions. We prove that the new metrics are complete and show useful relationships with $f$-divergences for probability distributions. To further extend our approach to structured objects such as concept hierarchies and ontologies, we introduce information-theoretic metrics on directed acyclic graphs drawn according to a fixed probability distribution. We conduct empirical investigation to demonstrate intuitive interpretation of the new metrics and their effectiveness on real-valued, high-dimensional, and structured data. Extensive comparative evaluation demonstrates that the new metrics outperformed multiple similarity and dissimilarity functions traditionally used in data mining, including the Minkowski family, the fractional $L^p$ family, two $f$-divergences, cosine distance, and two correlation coefficients. Finally, we argue that the new class of metrics is particularly appropriate for rapid processing of high-dimensional and structured data in distance-based learning.

==> discussion_ontology_distance.tex <==
\subsection{Dissimilarities for learning with ontologies}
In several recent publications non-metric similarity functions have been used to reason about functional similarity between biological macromolecules as well as prediction accuracy of automated annotation tools. Assuming non-empty sets $A$ and $B$, these include the Maryland bridge distance
% \[
% d_{\textrm{MB}}(A,B)=1-\left(\frac{1}{2}\frac{|A\cap B|}{|A|}+\frac{1}{2}\frac{|A\cap B|}{|B|}\right)
% \]
\[
d_{\textrm{MB}}(A,B)=1-\frac{1}{2}\left(\frac{|A\cap B|}{|A|}+\frac{|A\cap B|}{|B|}\right)
\]
\noindent where the term in the parentheses corresponds to the the Maryland bridge coefficient \citep{Glazko2005}. When $A$ is interpreted as a predicted set of terms for a protein and $B$ as a true set of terms, the Maryland bridge coefficient is simply an average of precision ($\nicefrac{|A\cap B|}{|A|}$) and recall ($\nicefrac{|A\cap B|}{|B|}$). Similarly, an often-used harmonic mean between precision and recall, referred to as F-measure \citep{Tan2006}, leads only to a near-metric called the Czekanowsky-Dice distance \citep{book}. This distance function can be expressed as
% \[
% d_{\textrm{CD}}(A,B)=1-\left(\frac{1}{2}\frac{|A|}{|A\cap B|}+\frac{1}{2}\frac{|B|}{|A\cap B|}\right)^{-1}
% \]
% \begin{align*}
% d_{\textrm{CD}} & =1-\left(\frac{1}{2}\frac{|A|}{|A\cap B|}+\frac{1}{2}\frac{|B|}{|A\cap B|}\right)^{-1} \\
% &=1-\frac{2|A\cap B|}{|A|+|B|}
% \end{align*}
% \begin{align*}
% d_{\textrm{CD}} & =1-2\Big((|A\cap B|/|A|)^{-1}+(|A\cap B|/|B|)^{-1}\Big)^{-1}\\
% &=1-\frac{2|A\cap B|}{|A|+|B|}
% \end{align*}
\begin{align*}
d_{\textrm{CD}} & =1-2\Big((|A\cap B|/|A|)^{-1}+(|A\cap B|/|B|)^{-1}\Big)^{-1}=1-\frac{2|A\cap B|}{|A|+|B|}
\end{align*}
\noindent where, again, $A$ and $B$ are sets and the second term on the right-hand side is the F-measure; more precisely, $F_1$ (observe here the similarity to Jaccard distance that loses the constant factor and has $|A \cup B|$ in the denominator). While on the surface the process of finding an average pairwise distance for a set of graphs appears to be straightforward, it is unclear what the effect of such operations might be when the concept of triangle inequality is violated. We therefore caution the interpretation of results when non-metric distance functions are used.


==> ontology_background.tex <==

\section{Learning with hierarchical object descriptors}
Modern machine learning approaches increasingly rely on hierarchical object descriptions. A news article, for instance, covering aspects of sports injuries might be labeled by the term ``sports'', ``medicine'', but also ``sports medicine'' that is a subcategory of both sports and medical articles. Similarly, a protein associated with the terms ``transferase'' and ``oxidoreductase'' could also be associated with a more general term ``enzyme''. While learning with such output spaces can be addressed via binary or multilabel strategies, it is often beneficial to also consider the relationships between the concepts (e.g., $\mathsf{is}$-$\mathsf{a}$, $\mathsf{part}$-$\mathsf{of}$). Unfortunately, hierarchical representations often have extremely large cardinality and, thus, require the development of distance functions that can provide necessary degrees of similarity between class labels. In this work we consider one special case of hierarchical representations that is generally referred to as ontologies.

An ontology $\mathcal{O}=(V,E)$ is a directed acyclic graph with a set of vertices (concepts, terms) $V$ and a set of edges (relational ties) $E\subset V\times V$. In terms of class labels, a news article or a protein function can be seen as a \emph{consistent subgraph} $F\subseteq V$ of the larger ontology graph. By saying consistent, we mean that if a vertex $v$ belongs to $F$, then all the ancestors of $v$ up to the root(s) of the ontology must also belong to $F$. Typically, a subgraph $F$ corresponding to an object such as experimentally characterized protein contains 10-100 nodes, whereas the ontology graph consists of 1000-10000 nodes. One example of such annotation is illustrated in Figure \ref{fig:ontology}. 

Although ontological representations have been considered in text mining \citep{Grosshans2014} and computer vision \citep{Movshovitz2015}, they have been arguably most well-developed in the biomedical sciences  \citep{Robinson2011}. The most frequently used ontology for the description of protein function is the Gene Ontology \citep{Ashburner2000}. Gene Ontology (GO) consists of three directed acyclic graphs describing different aspects of a protein's activity: the Molecular Function Ontology (MFO) describes protein function at the biochemical level; the Biological Process Ontology (BPO) provides a more abstract view in terms of the emergent biological processes a protein is involved in; and the Cellular Component Ontology (CCO) describes the location in or outside the cell where the protein carries out its function. 

\begin{figure}
\begin{centering}
%\includegraphics[scale=0.7]{ontology.pdf}
\includegraphics[scale=0.9]{ontology.pdf}
%\includegraphics[width=0.9\columnwidth]{ontology.pdf}
\par\end{centering}

\protect\caption{Illustration of a protein's functional annotation using the Biological Process Ontology. The functional annotation graph (blue nodes) contains two leaf nodes, `Lateral growth' and `Isotropic cell growth', that completely determine the consistent subgraph. All edges in the graph are $\mathsf{is}$-$\mathsf{a}$ and are read from child to parent. \label{fig:ontology}}
\end{figure}

\section{Comparing ontological annotations}
Similarity functions between pairs of consistent subgraphs can be broadly divided into topological and probabilistic.

Topological comparisons are usually node-based or edge-based, but can also incorporate the structure of the ontology. Similarity functions such as \cite{Jaccard} coefficient and cosine similarity are based on the sets of terms with which the two objects are annotated. More complex functions incorporate shortest path-based distances \citep{Rada1989}, node reachability \citep{Mazandu2012}, and others. While simple and generally interpretable, many of these functions do not adequately address the hierarchical nature of ontological terms or practical issues such as those related to the unequal specificity of these terms in different parts of the ontology. 

Probabilistic or information-theoretic similarity measures, on the other hand, incorporate the structure of the ontology but also assume an underlying probabilistic model for the data, where a ground truth database is used to estimate parameters of the model. Probabilistic similarity functions often derive from the semantic similarity proposed by \cite{Resnik1995}. This measure uses a database of labeled objects to estimate the probability of every node $v\in V$ and then computes the similarity between nodes $u$ and $v$ as $s_{R}(u,v)=-\log P(w)$, where $w$ is the node from $(\mathrm{Ancestors}(u)\cup\{u\})\cap(\mathrm{Ancestors}(v)\cup\{v\})$ with the lowest probability. The deficiencies of Resnik's similarity have been widely discussed and have led to several modifications \citep{Jiang1997, Lin1998}. However, the main problem of applying these measures to subgraphs of the ontology containing multiple leaf terms, as in Figure \ref{fig:ontology}, has not been resolved in a principled manner. In comparing two consistent subgraphs that contain multiple leaf terms, various approaches generally resort to ad hoc techniques such as all-pair averaging and others \citep{Resnik1999, Lord2003, Verspoor2006}.
